Advanced Models for the OSPF Routing Protocol

We present two formal models for the OSPF routing protocol, designed for the model checker Uppaal. The first one is an optimised model of an existing model that allows to check larger network topologies. The second one is a specialised model for adjacency building, a complex subprocedure of OSPF, which is not part of any existing model and which is known to be vulnerable to cyber attacks. We illustrate how both models can be used to discover vulnerabilities in routing protocols.

==> eptcsdata.tex <==
\providecommand{\firstpage}{13}
\providecommand{\publicationstatus}{Clemens Dubslaff and Bas Luttik (Eds.):\\
Models for Formal Analysis of Real Systems (MARS 2022)\\
EPTCS 355, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.355.2}{10.4204/EPTCS.355.2}}
\pdfoutput=1

